Pretrained Language Models as Visual Planners for Human Assistance

In our pursuit of advancing multi-modal AI assistants capable of guiding users to achieve complex multi-step goals, we propose the task of "Visual Planning for Assistance (VPA)". Given a succinct natural language goal, e.g., "make a shelf", and a video of the user's progress so far, the aim of VPA is to devise a plan, i.e., a sequence of actions such as "sand shelf", "paint shelf", etc. to realize the specified goal. This requires assessing the user's progress from the (untrimmed) video, and relating it to the requirements of natural language goal, i.e., which actions to select and in what order? Consequently, this requires handling long video history and arbitrarily complex action dependencies. To address these challenges, we decompose VPA into video action segmentation and forecasting. Importantly, we experiment by formulating the forecasting step as a multi-modal sequence modeling problem, allowing us to leverage the strength of pre-trained LMs (as the sequence model). This novel approach, which we call Visual Language Model based Planner (VLaMP), outperforms baselines across a suite of metrics that gauge the quality of the generated plans. Furthermore, through comprehensive ablations, we also isolate the value of each component--language pre-training, visual observations, and goal information. We have open-sourced all the data, model checkpoints, and training code.

==> tables/main-results-vlamp.tex <==
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%


%

%
%
%
%
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cccccc@{}}
\toprule
\multicolumn{2}{l}{Dataset} & \multicolumn{2}{c}{Crosstask}                                    & \multicolumn{2}{c}{COIN}                                         \\ \midrule
\multicolumn{2}{l}{}        & \multicolumn{1}{l}{VLaMP}           & \multicolumn{1}{l}{DDN}    & \multicolumn{1}{l}{VLaMP}           & \multicolumn{1}{l}{DDN}    \\ \midrule
$l=1$                  & nAcc & \textbf{50.6 {\scriptsize ± 1.4}} & 33.4 {\scriptsize ± 0.5} & \textbf{45.2 {\scriptsize ± 0.8}} & 29.3 {\scriptsize ± 0.3} \\ \midrule
\multirow{3}{*}{$l=3$} & SR   & \textbf{10.3 {\scriptsize ± 0.4}} & 6.8 {\scriptsize ± 0.3}  & \textbf{18.3 {\scriptsize ± 0.1}} & 10.1 {\scriptsize ± 0.4} \\
           & mAcc           & \textbf{35.3 {\scriptsize ± 1.1}} & 25.8 {\scriptsize ± 0.5}  & \textbf{39.2 {\scriptsize ± 0.3}}  & 22.3 {\scriptsize ± 0.4} \\
           & mIOU           & \textbf{44.0 {\scriptsize ± 1.0}} & 35.2 {\scriptsize ± 0.6} & \textbf{56.6 {\scriptsize ± 0.5}}          & 32.2 {\scriptsize ± 0.6} \\ \midrule
\multirow{3}{*}{$l=4$} & SR   & \textbf{4.4 {\scriptsize ± 0.2}}  & 3.6 {\scriptsize ± 0.2}   & \textbf{9.0 {\scriptsize ± 0.3}}          & 7.0 {\scriptsize ± 0.3} \\
           & mAcc           & \textbf{31.7 {\scriptsize ± 1.0}} & 24.1 {\scriptsize ± 0.4} & \textbf{35.2 {\scriptsize ± 0.2}} & 21.0 {\scriptsize ± 0.4} \\
           & mIOU           & \textbf{43.4 {\scriptsize ± 0.9}}          & 37.0 {\scriptsize ± 0.4} & \textbf{54.2 {\scriptsize ± 0.5}}          & 37.3 {\scriptsize ± 0.3} \\ \bottomrule
\end{tabular}%
}
\caption{The (mean ± std. error of mean) of various planning metrics obtained using 5 runs with different random seed. 
%
Note that the action history and observations are provided using the output of the action segmentation model and hence are noisy compared to the ground truth history.
}
\label{tab:main-results-vlamp}
\end{table}



%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

==> tables/main-results.tex <==
%
%
%
\begin{table*}[]
\centering
%
\begin{tabular}{llccccccc}
\hline
\multirow{2}{*}{Dataset} &
  \multirow{2}{*}{model} &
  \multicolumn{1}{c|}{\textbf{$l=1$}} &
  \multicolumn{3}{c|}{$l=3$} &
  \multicolumn{3}{c}{$l=4$} \\ \cline{3-9} 
 &
   &
  \multicolumn{1}{c|}{\textbf{nAcc}} &
  \textbf{SR} &
  \textbf{mAcc} &
  \multicolumn{1}{c|}{\textbf{mIOU}} &
  \textbf{SR} &
  \textbf{mAcc} &
  \textbf{mIOU} \\ \hline
crosstask &
  P3LM(G,A) &
  30.48 {\scriptsize ± 0.61} &
  8.18 {\scriptsize ± 0.39} &
  27.6 {\scriptsize ± 0.64} &
  42.06 {\scriptsize ± 0.54} &
  4.14 {\scriptsize ± 0.18} &
  26.23 {\scriptsize ± 0.59} &
  43.59 {\scriptsize ± 0.48} \\
crosstask &
  P3LM(G,A,O) &
  \textbf{50.61 {\scriptsize ± 1.47}} &
  \textbf{10.31 {\scriptsize ± 0.44}} &
  \textbf{35.36 {\scriptsize ± 1.12}} &
  \textbf{44.07 {\scriptsize ± 1.06}} &
  \textbf{4.47 {\scriptsize ± 0.29}} &
  \textbf{31.71 {\scriptsize ± 1.04}} &
  43.49 {\scriptsize ± 0.96} \\
crosstask &
  DDN(G,A,O) &
  33.41 {\scriptsize ± 0.51} &
  6.81 {\scriptsize ± 0.33} &
  25.86 {\scriptsize ± 0.5} &
  35.26 {\scriptsize ± 0.62} &
  3.61 {\scriptsize ± 0.2} &
  24.16 {\scriptsize ± 0.43} &
  37.07 {\scriptsize ± 0.47} \\ \hline
coin &
  P3LM(G,A) &
  41.49 {\scriptsize ± 0.35} &
  17.3 {\scriptsize ± 0.13} &
  37.56 {\scriptsize ± 0.29} &
  56.47 {\scriptsize ± 0.21} &
  9.13 {\scriptsize ± 0.09} &
  34.19 {\scriptsize ± 0.27} &
  54.21 {\scriptsize ± 0.22} \\
coin &
  P3LM(G,A,O) &
  \textbf{45.2 {\scriptsize ± 0.83}} &
  \textbf{18.3 {\scriptsize ± 0.19}} &
  \textbf{39.28 {\scriptsize ± 0.3}} &
  56.67 {\scriptsize ± 0.53} &
  9.02 {\scriptsize ± 0.34} &
  \textbf{35.27 {\scriptsize ± 0.28}} &
  54.26 {\scriptsize ± 0.59} \\
coin &
  DDN(G,A,O) &
  29.3 {\scriptsize ± 0.39} &
  10.1 {\scriptsize ± 0.46} &
  22.33 {\scriptsize ± 0.41} &
  32.26 {\scriptsize ± 0.67} &
  7.09 {\scriptsize ± 0.39} &
  21.02 {\scriptsize ± 0.49} &
  37.36 {\scriptsize ± 0.34} \\ \hline
\end{tabular}%
%
\caption{The (mean ± std. error of mean) of various planning metrics obtained using 5 runs with different random seed. The letters in the parentheses specify what is provided to the planning model during training and prediction, where G="Goal description", A="Action history", O="Accompanying observation history". Note that the action history and observations are provided using the output of the action segmentation model and hence are noisy compared to the ground truth history.
 
}
\label{tab:main-results-2}
\end{table*}
